Robust Linear Regression: Optimal Rates in Polynomial Time

We obtain robust and computationally efficient estimators for learning several linear models that achieve statistically optimal convergence rate under minimal distributional assumptions. Concretely, we assume our data is drawn from a $k$-hypercontractive distribution and an $\epsilon$-fraction is adversarially corrupted. We then describe an estimator that converges to the optimal least-squares minimizer for the true distribution at a rate proportional to $\epsilon^{2-2/k}$, when the noise is independent of the covariates. We note that no such estimator was known prior to our work, even with access to unbounded computation. The rate we achieve is information-theoretically optimal and thus we resolve the main open question in Klivans, Kothari and Meka [COLT'18]. Our key insight is to identify an analytic condition that serves as a polynomial relaxation of independence of random variables. In particular, we show that when the moments of the noise and covariates are negatively-correlated, we obtain the same rate as independent noise. Further, when the condition is not satisfied, we obtain a rate proportional to $\epsilon^{2-4/k}$, and again match the information-theoretic lower bound. Our central technical contribution is to algorithmically exploit independence of random variables in the "sum-of-squares" framework by formulating it as the aforementioned polynomial inequality.

==> mysymbols_backup.tex <==
\newcommand{\tiln}{\widetilde{n}}
\newcommand{\tilp}{\widetilde{p}}
\newcommand{\widetildelta}{\widetilde{\delta}}
\newcommand{\tildelta}{\widetilde{\delta}}
\newcommand{\link}{\Phi}


\newcommand\matnorm[2]{\left|\!\left|\!\left| #1 \right|\!\right|\!\right|_{#2}}
\newcommand\norm[2]{\left|\!\left|#1 \right|\!\right|_{#2}}
\newcommand\trace[1]{\text{tr}\left(#1\right)}
\def\real{\mathbb{R}}
\def\Exp{\mathbb{E}}


% theorem type environments
\newtheorem{theorem}{Theorem}
\newtheorem{condition}{Condition}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[lemma]{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{claim}{Claim}


%SpaceSaving Lists
\newcommand{\squishlist}{
   \begin{list}{$\bullet$}
       { \setlength{\itemsep}{0pt}      \setlength{\parsep}{1pt}
       \setlength{\topsep}{1pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
       \setlength{\labelsep}{0.5em} } }

\newcommand{\squishenum}[1]{
   \begin{enumerate}[label=(#1\arabic*)]
       { \setlength{\itemsep}{0pt}      \setlength{\parsep}{3pt}
       \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
       \setlength{\labelsep}{0.5em} } }



% general symbols
\newcommand{\RF}{\mathbb{R}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\nn}{\nonumber} 
\newcommand{\paren}[1]{\left( #1 \right)}
\newcommand{\sqprn}[1]{\left[ #1 \right]}
\newcommand{\tlprn}[1]{\left\{ #1 \right\}}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\tr}[2]{\left<\left< #1 , #2 \right>\right>}
\newcommand{\trs}[2]{\left< #1 , #2 \right>}
\newcommand{\iprod}[2]{\left\langle #1 , #2 \right\rangle}
\newcommand{\inprod}[2]{\left\langle #1 , #2 \right\rangle}

\newcommand{\del}{\partial}
\newcommand{\dd}[2]{\frac{d#1}{d#2}}
\newcommand{\ddel}[2]{\frac{\del#1}{\del#2}}
\newcommand{\ddell}[2]{\frac{\del^2#1}{{\del#2}^2}}
\newcommand{\ddelll}[3]{\frac{\del^2#1}{{\del#2}{\del#3}}}
\newcommand{\beq}{\begin{eqnarray*}}
\newcommand{\eeq}{\end{eqnarray*}}
\newcommand{\beqn}{\begin{eqnarray}}
\newcommand{\eeqn}{\end{eqnarray}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\poly}{\text{poly}}

\def \bal#1\eal{\begin{align}#1\end{align}}
\def \bals#1\eals{\begin{align*}#1\end{align*}}

\newcommand{\hide}[1]{}
\newcommand{\oo}[1]{\frac{1}{#1}}
\newcommand{\eps}{\epsilon}
\newcommand{\evalat}[2]{\left.#1\right|_{#2}}
\newcommand{\ceil}[1]{\ensuremath{\left\lceil#1\right\rceil}}
\newcommand{\floor}[1]{\ensuremath{\left\lfloor#1\right\rfloor}}
\newcommand{\ontop}[2]{\overset{{\scriptsize #1}}{#2}}
\newcommand{\Perp}{\perp\!\!\!\perp}
\newcommand{\limsu}{\mathop{\overline{\mathrm{lim}}}}
\newcommand{\limin}{\mathop{\underline{\mathrm{lim}}}}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand{\map}{\mathop{\mathrm{map}}}
\newcommand{\powrs}[1]{\langle\!\langle #1 \rangle\!\rangle}
\newcommand{\polys}[1]{\langle #1 \rangle}
\newcommand{\contf}{\mathscr{C}}
%\newcommand{\trn}{^{{}^\intercal}} %operator transpose
\newcommand{\trn}{^\intercal} %operator transpose
%\newcommand{\trn}{^{{}^{\!\intercal}}} %operator transpose
\newcommand{\inv}{^{-1}} %inverse
\newcommand{\unit}{\boldsymbol{1}}
\newcommand{\zero}{\boldsymbol{0}}
\newcommand{\defeq}{\stackrel{\mathrm{def}}{=}}
\newcommand{\textonTop}[2]{\stackrel{\mathrm{#1}}{#2}}

\newcommand{\pleq}{~+\!=}
\newcommand{\chr}{\mathrm{\bs{1}\hspace{-3pt}I}} % characteristic function
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}

% function names
\newcommand{\zeros}{\mathrm{zeros}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\TR}{\mathrm{tr}}
\newcommand{\vol}{\mathrm{vol}}
\newcommand{\sgn}{\mathrm{sgn}}
\newcommand{\acos}{\mathrm{acos}}
\newcommand{\intr}{\mathrm{int}\,}
\newcommand{\extr}{\mathrm{ext}\,}
\newcommand{\dom}{\mathrm{dom}\,}
\newcommand{\conv}{\mathrm{conv}\hspace{1pt}}
\newcommand{\cone}{\mathrm{cone}\hspace{1pt}}


%probability & statistics symbols
\newcommand{\convd}{\overset{{\scriptsize d}}{\to}}
\newcommand{\convp}{\overset{{\scriptsize p}}{\to}}
\newcommand{\unif}{\mathrm{Uniform}}
\newcommand{\bern}{\mathrm{Bernoulli}}
\newcommand{\negbin}{\mathrm{NegBinom}}
\newcommand{\Binom}{\mathrm{Bin}}
\newcommand{\pois}{\mathrm{Poisson}}
%\newcommand{\ndistr}{\mathrm{Normal}}
\newcommand{\ndistr}{\mathrm{n}}
\newcommand{\Bdistr}{\mathrm{Beta}}
\newcommand{\Gdistr}{\mathrm{Gamma}}
% f(x) = \frac{1}{\beta^\alpha\Gamma(\alpha)}x^{\alpha-1}e^{-x/\beta}
\newcommand{\iGdistr}{\mathrm{InvGamma}} 
% f(x) = \frac{1}{\beta^\alpha\Gamma(\alpha)}x^{-\alpha-1}e^{-1/(\beta x)}
\newcommand{\MSE}{\mathrm{MSE}} 
\newcommand{\MAE}{\mathrm{MAE}} 
\newcommand{\ARE}{\mathrm{ARE}} 
\newcommand{\se}{\mathrm{se}} 

%\newcommand{\eg}{\mathrm{e.g.}} 
%\newcommand{\st}{\mathrm{s.t.}} 
%\newcommand{\ie}{\mathrm{i.e.}} 

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}
\newcommand{\tha}{\theta}
%\newcommand{\mexp}{\mathbb{E}}
%\newcommand{\mexp}[1]{\ensuremath{\text{{\bf E}$\left[#1\right]$}}}
\newcommand{\mexp}{\text{{\bf E}}}
\newcommand{\var}{\mathrm{Var}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\corr}{\mathrm{Cor}}
\newcommand{\bW}{\bs{W}}
\newcommand{\bw}{\bs{w}}
\newcommand{\bX}{\bs{X}}
\newcommand{\bx}{\bs{x}}
\newcommand{\bY}{\bs{Y}}
\newcommand{\by}{\bs{y}}
\newcommand{\bZ}{\bs{Z}}
\newcommand{\bz}{\bs{z}}
\newcommand{\Xbar}{\overline{X}}
\newcommand{\ev}{\mathrm{Ev}} %evidence
\newcommand{\pr}{\boldsymbol{\mathrm{P}}}
%\newcommand{\prob}{\mathrm{Pr}}


% embeddings
\newcommand{\embeds}[1]{\;\lhook\joinrel\xrightarrow{#1}\;}

%misc commands
\newcommand{\ds}{\displaystyle}
%\newcommand{\ts}{\textstyle}
\newcommand{\bs}{\boldsymbol}
\renewcommand{\th}{\ensuremath{^{\mathrm{th}}}~}

\usepackage{eso-pic}
\usepackage{xspace}
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\st{s.t\onedot} \def\St{\emph{S.t}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\iid{i.i.d}
\def\etal{\emph{et al}\onedot}
\makeatother

% Miscellaneous
\def\naive{na\"\i ve\xspace}
\def\naively{na\"\i vely\xspace}
\def\Naive{Na\"\i ve\xspace}
\def\Naively{Na\"\i vely\xspace}

\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\eqnref}[1]{(\ref{#1})}
\newcommand{\secref}[1]{Section \ref{#1}}
\newcommand{\chapref}[1]{Chapter \ref{#1}}
\newcommand{\thmref}[1]{Theorem \ref{#1}}


%\include{mathmacro}
\makeatletter
\newcommand{\bfgreek}[1]{\bm{\@nameuse{#1}}}
\makeatother

\newcommand{\ind}[1]{[\hspace{-1pt}[#1]\hspace{-1pt}] }
\newcommand{\todo}[1]{\textcolor{red}{TODO: #1}}
\newcommand{\red}[1]{\textcolor{red}{#1}}

\newenvironment{indentpar}[1]%
     {\begin{list}{}%
             {\setlength{\leftmargin}{#1}}%
             \item[]%
     }
{\end{list}}

\makeatletter
\newcounter{problem}
\newenvironment{problem}[1][]{\refstepcounter{problem}\par\noindent%
\textbf{Problem~\theproblem: #1}}
%\textbf{Problem~\theproblem: #1}\rmfamily}
\makeatother



==> name.tex <==
%!TEX root = main.tex


Briefly, our algorithm simply does the following: 
\begin{enumerate}
  \item \textbf{Clustering via SoS}: Run Algorithm \ref{algo:robust-partial-clustering} repeatedly till the SDP is infeasable to obtain a partition of the samples, $\{\tilde{Y}_j\}_{j \in [t]}$, for some $t\in[k]$.

  \item \textbf{Robust Isotropic Transformation}: Run the algorithm corresponding to Lemma \ref{lem:sampling_from_nearl_isotropic} on each set $\tilde{Y}_j$ to make the sample approximately isotropic.
  \item \textbf{List-Decoding via Tensor Decomposition}:  Run Algorithm \ref{algo:list-recovery-tensor-decomposition} on each $\tilde{Y}_j$. Concatenate the lists to obtain $\calL$.
   \item \textbf{Robust Tournament}: Run the tournament from Fact~\ref{lem:tournament} over all the hypothesis in $\calL$, and output the winning hypothesis. 
\end{enumerate}

\paragraph{Correctness.}
Setting $\Delta = 1/k^2$, it follows from Theorem \ref{thm:partial-clustering} that we obtain a partition of $Y$ into $\{\tilde{Y}_j\}_{j \in [t]}$, for some $t\in[k]$ such that $\tilde{Y}_j$ has at most $\bigO{k^2\epsilon}$ outliers, $\Paren{1-\bigO{k^2\epsilon}}$-fraction of samples from at least $1$ component of the input mixture and the resulting samples are not $\bigO{1/k^2}$-separated. It then follows from Lemma \ref{lem:sampling_from_nearl_isotropic} that the mean $\mu_j$ and covariance $\Sigma_j$ of $\tilde{Y}_j$ satisfy : a) $\Norm{\mu_j}_2 \leq \bigO{ \sqrt{\epsilon k^4}} $, b)$\Paren{1- \sqrt{\epsilon}k^3 } I \preceq \Sigma_j\preceq \Paren{1- \sqrt{\epsilon}k^3 } I$ and c)$\Norm{\Sigma - I }_F \leq \bigO{\sqrt{\epsilon}k^3}$. 

A partition $\tilde{Y}_j$ can have at most $k$ components. Assuming these correspond to $\{\mu^{(j)}_i \Sigma^{(j)}_i \}_{i \in [k]}$, observe, $\frac{1}{k}\sum_{i \in[k]} \Sigma_i + \mu_i \mu_i^\top \preceq \Paren{1- \sqrt{\epsilon}k^3 } I$. Thus $\Norm{\mu_i}^2_2 \leq \Paren{1- \sqrt{\epsilon}k^3 }/k$ and  combined with not being $\bigO{1/k^2}$-separated, it follows that \Anote{editing here.}



We run full clustering and tensor decomposition, we get a lower bound in lowner ordering on each covariance of 1/poly(k) to poly(k) and also a poly(k) for Frobenius error. then isotropize to apply tensor decomposition and we immediately get tv closeness since we have additive Frobenius + lower bound on eigenvalues. 

==> old_content.tex <==





\paragraph{Setup.} Let $\calP_{2k}^{\tau_u,\tau_\ell}$ be the class of distributions with bounded $2k$-moments such that the covariance matrix $\tau_\ell I_p \preceq \Sigma(P) \preceq \tau_u I_p$, where we say that a random variable $x$ has bounded $2k$ moments if,
\[ \Exp[\paren{\inprod{v}{x - \Exp[x]}}^{2k}] \leq C_{2k} \paren{\Exp[\paren{\inprod{v}{x - \Exp[x]}}^2]}^{k} \]
Note that the above condition is also called $k$-hypercontractivity in the TCS community. To begin, we first define the class of distributions represented by a linear regression model $\calP_{\text{linreg},{2k}}^{\sigma^2,\tau_u,\tau_\ell}$
\begin{align*}
    & \calP_{\text{linreg},{2k}}^{\sigma^2,\tau_u,\tau_\ell} = \{  (x,y) \sim P_\theta~| \\ \Exp[x] = 0,
   & x \in \calP_{2k}^{\tau_u,\tau_\ell}, \\
   & \Exp[y - x^T \theta] = 0, ~y- x^T \theta(P) \sim \calP_{2k}^{\sigma^2,0}, \\
  &  z = y - x^T \theta(P) || x \}
\end{align*}
Note that the above class of distributions simply represents the data generation process where the covariates $x \sim \real^p$ are drawn from some zero-mean distribution $P_x  \in \calP_{2k}$ with covariance $\Sigma$ and the response $y \in \real$ is generated by,
\[ y = x^T \theta^* + w, \]
where $w$ is a zero mean noise random variable with variance $\sigma^2$ and bounded $2k$ moments. 

We work in the Huber Contamination model, \ie we observe samples $\calD_n = \{ x_i,y_i \}_{i=1}^n$ from $P_\epsilon$ given by
\[ P_\epsilon = (1- \epsilon) P^* + \epsilon Q ,\]
where $Q$ is an arbitrary distribution and $P^* \in \calP_{\text{linreg},{2k}}^{\sigma^2,\tau_u,\tau_\ell}$. Then, given these contaminated samples, the goal is to estimate $\theta^*$. Then, the goal is to design estimators which recover the true parameter $\theta(P)$.

\paragraph{Related Work.} There are only two known estimators~\cite{prasad2018robust,diakonikolas2018sever,kothari2018robust} for this general setting of linear regression.~\cite{prasad2018robust} and~\cite{diakonikolas2018sever} use a robust gradient based approach, and derive efficient estimators for the case when $k=2$. They obtain an asymptotic rate of $\norm{\eparam - \theta^*}{2} = O(\sigma \sqrt{\epsilon})$. Note that this translates to an excess prediction error of $O(\sigma^2 \epsilon)$. On the other hand, \cite{kothari2018robust} used an SOS construct a polynomial time estimator $\eparam_{\text{SOS}}$, which, under the assumption that $X$ has \emph{certifiably} bounded $2k_1$-moments($k_1 \geq 2$) has an excess prediction error of $O(\sigma^2 \epsilon^{1 - 1/k_1)}$ (See Theorem~5.1 in~\cite{kothari2018robust}).

Comparing the results for $k_1=2$, the gradient based estimators work give an $O(\sigma^2 \epsilon)$ excess prediction error, while SOS-based estimators give an excess prediction error of $O(\sigma^2 \sqrt{\epsilon})$. Surprisingly,~\cite{kothari2018robust} also provide a lower bound of $\Omega(\sqrt{\epsilon})$ on the prediction error.(See Lemma 6.2 in~\cite{kothari2018robust}).

\paragraph{Goal.} In this short note, we aim to study parameter recovery in robust linear regression. Our goals are three fold -- (1) Review existing work and reconcile the conflicting upper and lower bounds. (2) Construct exponential-time statistically optimal estimators for this setting. Note that one can always claim that doing a TV projection (or a relaxed version~See~\cite{zhu2019generalized}) will be optimal, but doing TV-projection requires constructing a TV-cover of distribution classes, but it is not clear on how to construct covers for such classes. (3) Use SOS to construct polynomial time estimators for distributions with certifiably bounded distributions.

\paragraph{Upper Bounds via Gradient Based Estimator.} Following the analysis of~\cite{prasad2018robust}, we know that at any point $\theta^{t}$, the gradient vector($\calG(\theta^t)$) has bounded $k$-moments if $X$ has bounded $2k$ moments and $w$ has bounded $2k$ moments, with the variance upper bounded by $\sigma^2\tau_u(\Sigma) + C_4 \norm{\Delta^t}{2}^2 \tau_u^2$, where $\Delta^t = \norm{\theta^t - \tparam}{2}$. Hence, if we do an information-theoretic optimal robust estimation of the gradient(See~\cite{prasad2019unified}), we can return an estimate $\widehat{G}(\theta^t)$, which comes with the following guarantee.
\begin{proposition}~\label{prop:robgrad}
When X and noise are zero mean and have bounded $2k$-moments and the covariance of X is $ \tau_\ell \calI_p \preceq \Sigma \preceq \tau_u \calI_p$  and the noise has variance $\sigma^2$. Then for \red{$k \geq 2$} and \red{$\epsilon \ll (\frac{1}{2 \kappa})^{\frac{k}{k-1}}$} robust gradient estimation returns an estimate such that,
\[ \norm{\eparam - \tparam}{2} \leq O \paren{\frac{\sigma}{\sqrt{\tau_\ell}} \epsilon^{1-1/k} \red{\sqrt{\frac{\tau_u}{\tau_\ell}}}}   \]
\end{proposition}
\begin{proof}[Proof Sketch]
\[ \norm{\hat{G}(\theta^t) - \calG(\theta^t)}{2} \leq \sigma \sqrt{\tau_u(\Sigma)} \epsilon^{1 - 1/k} + C_4 \norm{\Delta}{2} \tau_u \epsilon^{1 - 1/k} + O(1/\sqrt{n}) \]

Now, if we do gradient descent with these robust gradients, we get that for $\theta^{t+1} = \theta^t - \eta \hat{g}^t$ for $\eta = \frac{2}{\tau_\ell + \tau_u}$ we have that(See Theorem~1~\cite{prasad2018robust})
\[ \norm{\theta^{t+1} - \tparam}{2} \leq \sqrt{1 - \eta \frac{2\tau_\ell \tau_u}{\tau_\ell + \tau_u}} \norm{\Delta^t}{2} +  +  \eta \tau_u \norm{\Delta}{2} \epsilon^{1 - 1/k}  + \eta \sigma \sqrt{\tau_u(\Sigma)} \epsilon^{1 - 1/k}, \]
Collecting the terms together, we get that,
\[ \Delta^{t+1} \leq \underbrace{(1 - \frac{2 \tau_\ell - 2{\tau_u \epsilon^{1-1/k}}}{\tau_u + \tau_\ell})}_{\kappa} \Delta^{t-1} + 2 \eta \sigma \sqrt{\tau(\Sigma)} \epsilon^{1-1/k} \]
   Hence, as long as $\kappa < 1$, we have that
   \[ \norm{\Delta^{T+1}}{2} \leq \kappa^T \norm{\tparam}{2} + \frac{2 \eta \sigma \sqrt{\tau_u}}{1 - \kappa } \epsilon^{1-1/k} \]
   Observe that $\kappa = 1 - \eta (\tau_\ell - {\tau_u} \epsilon^{1- 1/k})$. Plugging this above, we get that,
    \[ \norm{\Delta^{T}}{2} \leq \kappa^{T} \norm{\Delta^0}{2} + \frac{\sigma \sqrt{\tau_u} \epsilon^{1-1/k}}{\tau_\ell - {\tau_u} \epsilon^{1- 1/k}}. \]
    Hence, as long as $\epsilon \ll \paren{\frac{1}{2\kappa}}^{\frac{k}{k-1}}$, one can get $O(\sigma \frac{\sqrt{\tau_u}}{\tau_\ell} \epsilon^{1-1/k})$ error rate in parameter recovery, which implies a excess prediction error of $O(\frac{\sigma^2}{\tau_\ell^2} \tau_u^2 \epsilon^{2-2/k})$. \\
\end{proof}

\paragraph{Lower Bound.}~\cite{kothari2018robust} have a lower bound in their paper but the lower bound confounds condition number and contamination level $\epsilon$, which doesn't provide the lower bound. Below, we present a cleaner lower bound.

\begin{lemma}\label{lem:lowerBound}
For $k=2$
\[ \omega_{TV}(\tparam(P),\calP_{\text{linreg},{2k}}^{\sigma^2,\tau_u,\tau_\ell}) = \sup \limits_{ \substack{{P_1,P_2 \in \calP_{\text{linreg},{2k}}^{\sigma^2,\tau_u,\tau_\ell}} \\ {TV(P_1,P_2) \leq \epsilon}}} \norm{\tparam(P_1) - \tparam(P_2)}{2} \geq \frac{\sigma \sqrt{\epsilon}}{\sqrt{\tau_\ell}}      \]
\end{lemma}

Comparing Proposition~\ref{prop:robgrad} and Lemma~\ref{lem:lowerBound}, we see that there exists a condition number gap in performance. Below, we present some comments, and question.


\apcomment{The general lower bound I think is $\Theta \paren{\frac{\sigma \epsilon^{1 - 1/k}}{\sqrt{\tau_\ell}}}$}


\bit 
\item \textbf{Question 1.} Suppose we assume that the $X's$ are isotropic \ie $\Sigma = \calI_p$, even then we don't have an estimator which gets the $O( \sigma \epsilon^{1-1/k})$ rate in parameter error. In exponential time, we know how to get it, but for \emph{certifiable} distributions there is no SOS method which gets the above rate in poly-time. 
\bit 
\item Is it the case that Pravesh's analysis can be improved?
\item I guess not. I think they're not solving the correct problem. In particular, they don't enforce the moment conditions on the covariates.
\item I believe that the solution is to stitch Pravesh's moment estimation paper's SOS constraints with his regression paper constraints. 
\eit 
\item \textbf{Question 2.} For the more general case, it is unclear on how to even construct exponential time but statistically optimal estimators.
\eit



% In this section, we show that bounded $2k$ moments suffice for obtaining an estimator that achieves optimal rate for outlier robust regression. 

% \begin{definition}($2k$-certifiable $c$-hypercontractivity.)
% A distribution $D$ is $k$-certifiably $c$-hypercontractive if for all $r\leq k$, there exists a degree-$2k$ sum-of-squares proof of the following inequality :
% \begin{equation*}
%     \expecf{x \sim D}{\langle x , v\rangle^{2r}} \leq  \left( c(r)\expecf{x\sim D}{ \langle x, v \rangle^2} \right)^{r}
% \end{equation*}
% \end{definition}



% \begin{lemma}
% Let $(X,Y) \in \mathbb{R}^{n\times d} \times \mathbb{R}^n$.  
% Let $D,D'$ be two distributions over $(X,Y)$ such that $\norm{D - D'}{TV} \leq \epsilon$. Moreover, suppose that $D_X,D'_X$~\footnote{They are the marginals over the covariates} be $2k$-certifiably $c$-hypercontractive.
% %moments. 
% Let $\tparam(D) = \argmin \limits_{\theta} \Exp_{(x,y) \sim D} [(y - x^T \theta)^2]$, similarly let $\tparam(D') = \argmin \limits_{\theta} \Exp_{(x',y') \sim D'} [(y' - (x')^T \theta)^2]$. Moreover, let $D,D'$ be such that for $(x,y) \sim D$, $y-x^T \tparam(D)$ has bounded $2k$-moments with variance $\sigma^2(D)$ and let $\Sigma(D)= \expecf{x\sim D_X}{xx^{\top}}$. Then, we have that
% \[ \norm{\tparam(D)- \tparam(D')}{2} \leq  O \left( \frac{\sigma(D)}{\sqrt{\tau_{\min}(\Sigma(D))}} \epsilon^{1-1/k}\right) \]
% %O \left( \frac{\sigma(D)}{(1 - \epsilon^{1-1/k}) \sqrt{\tau_{\min}(\Sigma(D))}} \epsilon^{1-1/k}\right)
% \end{lemma}
% % \apcomment{Think of D as the clean and nice distribution \ie equal mass on inliers.} \\
% % \apcomment{Think of D' as some points which you chose. Note I'm only imposing moment constraints on D'}. 
% \todo{Verify proof and lemma once more. Think about just prediction error.}
% \begin{proof}
% Note that since $\tparam(D) = \argmin_{\theta} \Exp_{(x',y') \sim D}[(y'-(x')^T \theta)^2]$, hence, we have that
% \begin{align}
%     \Exp_{(x,y)\sim D}[(v^T x) ((x)^T \tparam(D) - y)] = 0~~ \mid \forall v ~~\text{\red{Just the gradient condition}}
% \end{align}
% Now, let $\calG$ be the maximal coupling of $D,D'$ over $(x,y) \times (x',y')$. Then, we have that
%  \begin{equation*}
%  \begin{split}
%   \underbrace{\Exp_{\calG}[(v^T x)((x)^T \tparam(D) - y)]}_{=0} & = \Exp_{\calG}[(v^T x)((x)^T \tparam(D) - y) \indic{(x,y) == (x',y')}] \\
%   & +  \Exp_{\calG}[(v^T x)((x)^T \tparam(D) - y) \indic{(x,y) \neq (x',y')}] \\
%  \end{split}
% \end{equation*}
% Further, observe $\Exp_{\calG}[ v^T(x')( x'^T \tparam(D) - y' ) \indic{(x,y) == (x',y'))} ] \leq \Exp_{\calG}[ v^T(x')( x'^T \tparam(D) - y' )]$. Therefore, we have 
% \begin{equation*}
%     \begin{split}
%         0 & \leq \Exp_{\calG}[ v^T(x')( x'^T \tparam(D) - y' )] + \Exp_{\calG}[(v^T x)((x)^T \tparam(D) - y) \indic{(x,y) \neq (x',y')}] \\
%     \end{split}
% \end{equation*}
% \TODO{We now want to upper bound $\Exp_{\calG}[ v^T(x')( x'^T \tparam(D) - y' )]$ in terms of $\tparam(D) - \tparam(D')$ using a low degree proof. } Now, by Holder's Inequality, we have 
% \begin{equation*}
% \begin{split}
%     \Exp_{\calG}[(v^T x)((x)^T \tparam(D) - y) \indic{(x,y) \neq (x',y')}] & \leq \Exp_{\calG}\left[\indic{(x,y) \neq (x',y')}\right]^{1- \frac{1}{k}} \paren{ \Exp_{\calG}[(v^T x)^k(x^T \tparam(D) - y)^k]}^{1/k} \\
%     & \leq \epsilon^{1-\frac{1}{k}} \paren{ \Exp_{\calG}[(v^T x)^k(x^T \tparam(D) - y)^k]}^{1/k}
% \end{split}
% \end{equation*}
% Combining the two equations above, we have 
% \begin{equation*}
%     \begin{split}
%         %0 & \leq v^T \Sigma(D') (\tparam(D)-\tparam(D')) + \Exp_{\calG}[(v^T x)((x)^T \tparam(D) - y) \indic{(x,y) \neq (x',y')}] \\
%   v^T \Sigma(D') (\tparam(D)-\tparam(D')) & \leq    \epsilon^{1-1/k} \paren{ \Exp_{\calG}[(v^T x)^k(x^T \tparam(D) - y)^k]}^{1/k}
%     \end{split}
% \end{equation*}
% Using Cauchy-Schwartz to control the RHS, we get that, 
%  \[ \paren{ \Exp_{\calG}[(v^T x)^k(x^T \tparam(D) - y)^k]} \leq \sqrt{\Exp_{\calG}[(v^T x)^{2k}]} \sqrt{\Exp_{\calG}(x^T \tparam(D) - y)^{2k}}  \]
%  \apcomment{Note that if $D$ was such that $(y - x^T \tparam(D))$ was independent of x, then I need not do cauchy schwartz?, In any case let's proceed.}
% Plugging $v^T = v^T \Sigma(D)^{-\half}$, we get that 
% \[ v^T \Sigma(D)^{-\half} \Sigma(D') (\tparam(D') - \tparam(D)) \leq \epsilon^{1-1/k} \sqrt{v^T v} \sigma(D),  \]
% where $\sigma^2(D) = \var_D(y - x^T \tparam(D))$ is the variance of the noise process for $D$.
% Setting $v = \frac{\tparam(D') - \tparam(D)}{\norm{\tparam(D') - \tparam(D)}{2}}$, we get that
% \[ \frac{(\tparam(D') - \tparam(D))^T \Sigma(D)^{-\half} \Sigma(D') (\tparam(D') - \tparam(D))}{\norm{\tparam(D') - \tparam(D}{2}} \leq \sigma(D) \epsilon^{1-1/k}  \]


% Now, we know that since $D,D'$ are close in TV and $D_x,D'_x$ have bounded $2k$-moments, hence, we have that,
% \[ (1 - \epsilon^{1-1/k})\Sigma(D) \preceq \Sigma(D') \preceq \Sigma(D) (1 + \epsilon^{1-1/k}) \]
% Then, we get that, $(1- \epsilon^{1-1/k}) \Sigma(D)^{\half} \preceq \Sigma(D)^{-\half} \Sigma(D')$. Plugging this above, we get that, 
% \[ (1 - \epsilon^{1-1/k}) \sqrt{\tau_{\min}(\Sigma(D))} \norm{\tparam(D') - \tparam(D)}{2} \leq \sigma(D) \epsilon^{1-1/k} \]
% Hence, we get that
% \[ \norm{\tparam(D') - \tparam(D)}{2} \leq \frac{\sigma(D)}{(1 - \epsilon^{1-1/k}) \sqrt{\tau_{\min}(\Sigma(D))}} \epsilon^{1-1/k}  \]
% \end{proof}

% \paragraph{Proof for optimal error.} The proof is exactly the same I think. Note that from the above analysis, we have that for any vector $v$, 
% \begin{align}
%     v^T \Sigma(D') (\tparam(D') - \tparam(D)) &= \Exp_{\calG}[(v^T x)((x)^T \tparam(D) - y) \indic{(x,y) \neq (x',y')}] \nonumber \\
%   & \leq \epsilon^{1-1/k} \paren{ \Exp_{\calG}[(v^T x)^k(x^T \tparam(D) - y)^k]}^{1/k} \nonumber \\
%   & \leq \sigma(D) \epsilon^{1-1/k} \sqrt{v^T \Sigma(D) v} \label{eqn:bb1}
% \end{align}
% Moreover, since $D,D'$ are such that the marginals over the covariates $X$ are $2k$-hypercontractive, hence, we have that,
% \[ (1 - \epsilon^{1-1/k}) \Sigma(D) \preceq \Sigma(D') \preceq (1 + \epsilon^{1-1/k}) \Sigma(D) \]
% Hence, for any vector $v$, we have that,
% \[ (1-\epsilon^{1-1/k})v^T \Sigma(D) v \leq v^T \Sigma(D') v \]
% Substituting $v = (\tparam(D') - \tparam(D))$ in \eqref{eqn:bb1}, we get that
% \begin{align}
%     (1 - \epsilon^{1-1/k}) v^T\Sigma(D) v \leq \sigma \epsilon^{1-1/k} \sqrt{v^T \Sigma(D) v}
% \end{align}
% Henc, we get that,
% \[ \norm{\Sigma(D)^{\half}(\tparam(D') - \tparam(D))}{2} \leq \sigma \epsilon^{1-1/k} \]
% Note that the excess prediction error of $\tparam(D')$ \wrt to $D$, 
% \TODO{This step isn't clear to me, perhaps you can explain it.}
% \begin{align}
%      \text{err}_D(\tparam(D')) - \text{\err}_{D}(\tparam(D)) = \Exp_{(x,y) \sim D}[(y-x^T \theta)]
% \end{align}
% \[ \text{err}_D(\tparam(D')) - \text{\err}_{D}(\tparam(D)) = \norm{\Sigma(D)^{\half}(\tparam(D') - \tparam(D))}{2}^2 \]
% Hence, we get that
% \[ \text{err}_D(\tparam(D')) - \text{\err}_{D}(\tparam(D)) \leq \sigma^2 \epsilon^{2-2/k}  \]
% Hence, we don't get the minimum eigenvalue condition involved in the upperbound.




\clearpage
\section{Identifiability/Information Theoretic Proof[Corrected]}
I think the previous result had a bug. I think fixed it. But you should check.

\begin{lemma}
Let $(X,Y) \in \mathbb{R}^{d} \times \mathbb{R}$ and let $D,D'$ be two distributions over $(X,Y)$ such that $\norm{D - D'}{TV} \leq \epsilon$. Moreover, suppose that $D_X,D'_X$~\footnote{They are the marginals over the covariates} be $k$-certifiably $c$-hypercontractive.
%moments. 
Let $\tparam(D) = \argmin \limits_{\theta} \Exp_{(x,y) \sim D} [(y - x^T \theta)^2]$, similarly let $\tparam(D') = \argmin \limits_{\theta} \Exp_{(x',y') \sim D'} [(y' - (x')^T \theta)^2]$. Moreover, let $D,D'$ be such that for $(x,y) \sim D$, $y-x^T \tparam(D)$ is $k$-hypercontractive, with variance $\sigma^2(D)$ and let $\Sigma(D)= \E{x\sim D_X}{xx^{\top}}$. Then, we have that
\[ \norm{\Sigma(D')^{\half}(\tparam(D)-\tparam(D'))}{2} \leq O\paren{\sigma \epsilon^{1-1/k}}, \]
when the noise $y-x^T \tparam(D)$ is independent of $x$. Else, we have that, 
\[ \norm{\Sigma(D')^{\half}(\tparam(D)-\tparam(D'))}{2} \leq O\paren{\sigma \epsilon^{1-2/k}} \]
%O \left( \frac{\sigma(D)}{(1 - \epsilon^{1-1/k}) \sqrt{\tau_{\min}(\Sigma(D))}} \epsilon^{1-1/k}\right)
\end{lemma}
\begin{align*}
L_D(\theta^*(D')) - L_{D}(\theta^*(D)) = \Exp_{(x,y)\sim D}[(y- x^T \theta^*(D) + x^T \theta^*(D) - x^T \theta^*(D'))^2] - \Exp_{(x,y)\sim D}[(y-x^T \theta^*(D))^2]
\end{align*}
Put $y = x^T \theta^*(D) + (y - x^T \theta^*(D))$ in the first term. Based on which we get,
\[ L_D(\theta^*(D')) - L_{D}(\theta^*(D)) = \Exp_{(x,y)\sim D}[\Delta^T(xx^T) \Delta] + 2\Exp[(y - x^T \theta^*(D))(x^T \Delta )],  \]
where $\Delta = (\theta^*(D) - \theta^*(D'))$.

Before presenting the proof, observe that this directly gives a condition-number free bound for excess prediction error of $O(\sigma^2 \epsilon^{2-2/k})$ and is the first estimator to achieve this bound.
\begin{proof}
Note that since $\tparam(D) = \argmin_{\theta} \Exp_{(x',y') \sim D}[(y'-(x')^T \theta)^2]$, hence, we have that
\begin{align}
    \Exp_{(x,y)\sim D}[(v^T x) ((x)^T \tparam(D) - y)] = 0~~ \mid \forall v ~~\text{\red{Just the gradient condition}}
\end{align}
Now, let $\calG$ be the maximal coupling of $D,D'$ over $(x,y) \times (x',y')$. Then, we have that
 \begin{equation*}
 \begin{split}
   \underbrace{\Exp_{\calG}[(v^T x)((x)^T \tparam(D) - y)]}_{=0} & = \Exp_{\calG}[(v^T x)((x)^T \tparam(D) - y) \indic{(x,y) == (x',y')}] \\
   & +  \Exp_{\calG}[(v^T x)((x)^T \tparam(D) - y) \indic{(x,y) \neq (x',y')}] \\
 \end{split}
\end{equation*}
Hence, we have that,
\[ \underbrace{\abs{ \Exp_{\calG}[(v^T x)((x)^T \tparam(D) - y) \indic{(x,y) == (x',y')}]}}_{T1} = \underbrace{\abs{\Exp_{\calG}[(v^T x)((x)^T \tparam(D) - y) \indic{(x,y) \neq (x',y')}]}}_{T2} \]

\paragraph{Upperbounding T2.} We use Holder's inequality to upper bound T2.

\begin{align*}
T2 & \leq \Exp_{\calG}\left[\indic{(x,y) \neq (x',y')}\right]^{1- \frac{1}{k}} \paren{ \Exp_{\calG}[(v^T x)^k(x^T \tparam(D) - y)^k]}^{1/k} \\
    & \leq \epsilon^{1-\frac{1}{k}} \paren{ \Exp_{\calG}[(v^T x)^k(x^T \tparam(D) - y)^k]}^{1/k} \\
    & \leq C(k) \sigma(D) \epsilon^{1-\frac{1}{k}} \sqrt{v^T \Sigma(D) v}  
    \end{align*} 

\paragraph{Lowerbounding T1.}
Recall that $T1 = \Exp_{\calG}[(v^T x) (x^T \tparam(D) - y) \indic{(x,y) == (x',y')}]$.\red{This is where we made a mistake before.} Note that we have the following equation,
\begin{align*}
    \underbrace{\Exp_{\calG}[(v^T x') ((x')^T \tparam(D) - y')]}_{T3} & = \underbrace{\Exp_{\calG}[(v^T x) (x^T \tparam(D) - y) \indic{(x,y) == (x',y')}]}_{T5} \\ 
    & + \underbrace{\Exp_{\calG}[(v^T x') ((x')^T \tparam(D) - y') \indic{(x,y) \neq (x',y')}]}_{T4}
\end{align*}
Observe that $T1 = \abs{T5} = \abs{T3 - T4} \geq \abs{T3} - \abs{T4}$. Now, we write the explicit form for $T3$,
\[ T3 = \Exp_{\calG}[(v^T x') ((x')^T \tparam(D) - y')] = v^T \Sigma(D')(\tparam(D)-\tparam(D')) \]
Plugging this above, we get that, 
\begin{align}\label{eqn:1}
    \abs{v^T \Sigma(D')(\tparam(D)-\tparam(D'))} \leq \abs{T4} + T2
\end{align}
Next, we upper bound $\abs{T4}$, 

\paragraph{Upperbounding T4.}
 \begin{align*}
     T4 & = \Exp_{\calG}[(v^T x') ((x')^T \tparam(D) - y') \indic{(x,y) \neq (x',y')}] \\
     & = \Exp_{\calG}[(v^T x') ((x')^T \tparam(D) - (x')^T \tparam(D') + (x')^T \tparam(D') - y') \indic{(x,y) \neq (x',y')}] \\
     & = \underbrace{\Exp_{\calG}[(v^T x') ((x')^T \tparam(D) - (x')^T \tparam(D'))\indic{(x,y) \neq (x',y')}]}_{T4a} + \underbrace{\Exp_{\calG}[(v^T x') ((x')^T \tparam(D') - y') \indic{(x,y) \neq (x',y')}]}_{T4b}
 \end{align*}
 Note that $\abs{T4b}$ can be upperbounded similar to $T2$ using Holder's inequality, which gives us,
 \[ \abs{T4b} \leq  C(k) \sigma(D') \epsilon^{1-1/k} \sqrt{v^T \Sigma(D') v} \]
 Note that $T4a$, is given by, 
 \[ T4a = \Exp_{\calG}[(v^T (x'(x')^T) (\tparam(D) - \tparam(D')) \indic{(x,y) \neq (x',y')}] \]
 Substituting $v = (\tparam(D) - \tparam(D'))$, we get that,
 \[ T4a = \Exp_{\calG}[(v^T x')^2 \indic{(x,y) \neq (x',y')}] \]
 Hence, using Holder's we get that,
 \[ \abs{T4a} \leq \Exp_{\calG}[(v^T x')^{k}]^{2/k} \epsilon^{1-2/k} \leq C^2(k) v^T \Sigma(D') v (\epsilon^{1-2/k}) \]
Plugging our upper bounds on $\abs{T4}$ and $T2$ into~\eqref{eqn:1}, we get that $v = \tparam(D) - \tparam(D')$
\[  | v^T \Sigma(D') v | \leq C(k) \sigma(D) \epsilon^{1-1/k} \sqrt{v^T \Sigma(D) v} + C(k) \epsilon^{1-1/k}  \sigma(D') \sqrt{v^T \Sigma(D') v} + C^2(k) v^T(\Sigma(D'))v \epsilon^{1-2/k} \]
Hence, we get that,
\[ v^T \Sigma(D') v \paren{1 - C^2(k) \epsilon^{1-2/k}} \leq C(k) \sigma(D) \epsilon^{1-1/k} \sqrt{v^T \Sigma(D) v} + C(k) \epsilon^{1-1/k}  \sigma(D') \sqrt{v^T \Sigma(D') v} \]
The final step is to relate $v^T\Sigma(D)v$ to $v^T \Sigma(D') v$. This follows from the certifiable $k$-hypercontractivity of $D_x$ and $D'_x$. In particular, we know that since $D,D'$ are close in TV and $D_x,D'_x$ have bounded $k$-hypercontractivity, hence, we have that,
\[ (1 - \epsilon^{1-2/k})\Sigma(D') \preceq \Sigma(D) \preceq \Sigma(D') (1 + \epsilon^{1-2/k}) \]
Plugging this finally in the above equation, we get that,
\[ v^T \Sigma(D') v \paren{1 - C^2(k) \epsilon^{1-2/k}} \leq C(k) \epsilon^{1-1/k} \sqrt{v^T \Sigma(D') v} \paren{\sigma(D) \sqrt{1 + \epsilon^{1-2/k}} \sigma(D')} \]
Hence, we get that,
\[ \sqrt{v^T \Sigma(D') v} \leq O\paren{C(k) \sigma \epsilon^{1-1/k}} \]
Recall that $v = (\tparam(D) - \tparam(D'))$. Hence we get that,
\[ \norm{\Sigma(D')^{\half}(\tparam(D) - \tparam(D'))}{2} \leq  O\paren{C(k) \sigma \epsilon^{1-1/k}}. \]
Moreover recall that 
\begin{align}
     \text{err}_{D'}(\tparam(D)) - \text{\err}_{D'}(\tparam(D')) = \Exp_{(x',y') \sim D'}[(y'-(x')^T \tparam(D))^2] - \Exp_{(x',y') \sim D'}[(y'-(x')^T \tparam(D'))^2]
\end{align}
\[ \text{err}_{D'}(\tparam(D)) - \text{\err}_{D'}(\tparam(D')) = \norm{\Sigma(D')^{\half}(\tparam(D) - \tparam(D'))}{2}^2 \]
Hence, we get that
\[ \text{err}_D(\tparam(D')) - \text{\err}_{D}(\tparam(D)) \leq O\paren{C^2(k) \sigma^2 \epsilon^{2-2/k}}  \]
Hence, we don't get the minimum eigenvalue condition involved in the upperbound.
\end{proof}


\section{Lower Bound of \cite{kothari2018robust}.}
We consider the construction of the lower bound (Lemma~6.2) in \cite{kothari2018robust}. 

\paragraph{Setup.} Note that it a 2D example \ie $(x_1,x_2) \in \real^2$. Moreover note that the marginal distribution over $D_x$ and $D'_x$ are the same, and in particular the pdf is given by,
\begin{align}\label{eqn:dist_lb}
    D_x(x_1) = \begin{cases}
1/2 , ~~ \text{if} ~~ x_1 \in [-1,1] \\
0 ~~ \text{else} ~~
\end{cases} D_x(x_2) =  \begin{cases}
\delta/2 , ~~ \text{if} ~~ x_2 \in \{ -1/\delta^{1/4}, 1/\delta^{1/4} \} \\
\frac{(1 - \delta)}{2\eta} ~~ \text{else if} ~~ x_2 \in [-\eta,\eta], \\
0 ~~ \text{else} ~~
\end{cases}
\end{align}

Moreover, $\theta^*(D) = (1,1)$, and $\theta^*(D') = (1,-1)$. Hence, we have that 
\[ D(y | (x_1,x_2)) = x_1 + x_2 + \omega \] and \[D'(y | (x_1,x_2)) = x_1 - x_2 + \omega ,\]
where the noise $\omega \in \real$ is drawn uniformly over $[-\sigma,\sigma]$\footnote{They fix $\sigma$ to 1}. 

\paragraph{(4,c)-hypercontractivity.} Next, we calculate the hypercontractivity coefficient for the marginals of this distribution. In particular, we focus on the marginal over $x_2$ 
\[ \Exp[x_2^4] = \frac{(1-\delta)}{5} \eta^4 + \delta \cdot ( \frac{1}{\delta^{1/4}} )^4 = 1 + \frac{(1-\delta)}{5} \eta^4\]
\[ \Exp[x_2^2] = \frac{(1-\delta)}{3} \eta^2 + \delta \cdot ( \frac{1}{\delta^{1/4}} )^2  = \frac{(1-\delta)}{3} \eta^2 + \sqrt{\delta} \]
 Now note that $ (\Exp[x_2^2])^2 \leq 2(\delta + (1-\delta)^4/9 \eta^4)$, where as $\Exp[x_2^4]$ is an $O(1)$ term. Hence to find a constant such that,
 \[ (\Exp[x_2^4])^{1/4} \leq C(4) \sqrt{(\Exp[x_2^2])}, \]
 we need that $C(4)^4 \max(\delta,\eta^4) = \Omega(1)$
 This means that $C(4)$ will be an $\Omega(\min(1/\delta^{1/4},1/\eta))$ term. 

\paragraph{Excess Prediction Error.} First, we bound the excess error. Recall that the excess error is given by,
\begin{align}
\text{err}_{D'}(\tparam(D)) - \text{\err}_{D'}(\tparam(D')) = \Exp_{(x',y') \sim D'}[(y'-(x')^T \tparam(D))^2] - \Exp_{(x',y') \sim D'}[(y'-(x')^T \tparam(D'))^2]
\end{align}
which in this setting reduces to,
\[ \text{err}_{D'}(\tparam(D)) - \text{\err}_{D'}(\tparam(D')) = (0,2)^T \Sigma(D') (0,2) = 4 \Exp_{x_2 \sim D'}[x_2^2] = 4 \sqrt{\delta} + \frac{4\eta^2}{3} (1-\delta)  \]

\paragraph{Total Variation calculation.} Next, we calculate the total variation between the two distributions.


\begin{align*}
    TV(D,D') & = \half  \int_{(x_1,x_2,y)} \abs{D(x_1,x_2,y) - D'(x_1,x_2,y)} \\
    & = \half \int_{(x_1,x_2)} D_x(x_1,x_2) \int_y \abs{D(y|x_1,x_2)- D'(y|x_1,x_2)}
\end{align*}
Now, $D_1(y|x_1,x_2)$ is uniform over $[x_1+x_2-1,x_1+x_2+1]$. Similarly, $D_2(y | x_1,x_2)$ is uniform over $[x_1-x_2-1,x_1-x_2+1]$. So, the inner part of the intergral is equal to $2TV(\calU[x_1-x_2-\sigma,x_1-x_2+\sigma],\calU[x_1+x_2-\sigma,x_1+x_2+\sigma])$, \ie uniform distributions shifted by $2x_2$. 
\[ \int_y \abs{D_1(y|x_1,x_2)- D_2(y|x_1,x_2)} = 2 \indic{\abs{2 x_2} > 2\sigma} + \frac{\abs{2 x_2}\indic{\abs{2 x_2} \leq 2\sigma}}{\sigma} \]
Hence, we get that,
\[ TV(D_1,D_2) = \Pr(\abs{2 x_2} > 2\sigma) + \frac{\Exp_{2 x_2 \sim D_x}[\abs{2 x_2}\indic{\abs{2 x_2} \leq 2\sigma}]}{2\sigma} \]




% % \section{Lower Bound of \cite{klivans2018efficient}}
% % We consider the construction of the lower bound (Lemma~6.2) in \cite{klivans2018efficient}. 
% Note that it a 2D example \ie $(x_1,x_2) \in \real^2$. Moreover note that the marginal distribution over $D_x$ and $D'_x$ are the same, and in particular the pdf is given by,
% \begin{align}\label{eqn:dist_lb}
%     D_x(x_1) = \begin{cases}
% 1/2 , ~~ \text{if} ~~ x_1 \in [-1,1] \\
% 0 ~~ \text{else} ~~
% \end{cases} D_x(x_2) =  \begin{cases}
% \delta/2 , ~~ \text{if} ~~ x_2 \in \{ -1/\delta^{1/4}, 1/\delta^{1/4} \} \\
% \frac{(1 - \delta)}{2\epsilon \sigma} ~~ \text{else if} ~~ x_2 \in [-\epsilon \sigma,\epsilon \sigma], \\
% 0 ~~ \text{else} ~~
% \end{cases}
% \end{align}

% Moreover, $\theta^*(D) = (1,1)$, and $\theta^*(D') = (1,-1)$. Hence, we have that 
% \[ D(y | (x_1,x_2)) = x_1 + x_2 + \omega \] and \[D'(y | (x_1,x_2)) = x_1 - x_2 + \omega ,\]
% where the noise $\omega \in \real$ is drawn uniformly over $[-\sigma,\sigma]$\footnote{They fix $\sigma$ to 1}. 

% \paragraph{(4,c)-hypercontractivity.} Next, we calculate the hypercontractivity coefficient for the marginals of this distribution. In particular, we focus on the marginal over $x_2$ 
% \[ \Exp[x_2^4] = \frac{(1-\delta)}{5} \eta^4 + \delta \cdot ( \frac{1}{\delta^{1/4}} )^4 = 1 + \frac{(1-\delta)}{5} \eta^4\]
% \[ \Exp[x_2^2] = \frac{(1-\delta)}{3} \eta^2 + \delta \cdot ( \frac{1}{\delta^{1/4}} )^2  = \frac{(1-\delta)}{3} \eta^2 + \sqrt{\delta} \]
%  Now note that $ (\Exp[x_2^2])^2 \leq 2(\delta + (1-\delta)^4/9 \eta^4)$, where as $\Exp[x_2^4]$ is an $O(1)$ term. Hence to find a constant such that,
%  \[ (\Exp[x_2^4])^{1/4} \leq C(4) \sqrt{(\Exp[x_2^2])}, \]
%  we need that $C(4)^4 \max(\delta,\eta^4) = \Omega(1)$
%  This means that $C(4)$ will be an $\Omega(\min(1/\delta^{1/4},1/\eta))$ term. 

% \paragraph{Excess Prediction Error.} First, we bound the excess error. Recall that the excess error is given by,
% \begin{align}
% \text{err}_{D'}(\tparam(D)) - \text{\err}_{D'}(\tparam(D')) = \Exp_{(x',y') \sim D'}[(y'-(x')^T \tparam(D))^2] - \Exp_{(x',y') \sim D'}[(y'-(x')^T \tparam(D'))^2]
% \end{align}
% which in this setting reduces to,
% \[ \text{err}_{D'}(\tparam(D)) - \text{\err}_{D'}(\tparam(D')) = (0,2)^T \Sigma(D') (0,2) = 4 \Exp_{x_2 \sim D'}[x_2^2] = 4 \sqrt{\delta} + \frac{4\eta^2}{3} (1-\delta)  \]

% \paragraph{Total Variation calculation.} Next, we calculate the total variation between the two distributions.


% \begin{align*}
%     TV(D,D') & = \half  \int_{(x_1,x_2,y)} \abs{D(x_1,x_2,y) - D'(x_1,x_2,y)} \\
%     & = \half \int_{(x_1,x_2)} D_x(x_1,x_2) \int_y \abs{D(y|x_1,x_2)- D'(y|x_1,x_2)}
% \end{align*}
% Now, $D_1(y|x_1,x_2)$ is uniform over $[x_1+x_2-1,x_1+x_2+1]$. Similarly, $D_2(y | x_1,x_2)$ is uniform over $[x_1-x_2-1,x_1-x_2+1]$. So, the inner part of the intergral is equal to $2TV(\calU[x_1-x_2-\sigma,x_1-x_2+\sigma],\calU[x_1+x_2-\sigma,x_1+x_2+\sigma])$, \ie uniform distributions shifted by $2x_2$. 
% \[ \int_y \abs{D_1(y|x_1,x_2)- D_2(y|x_1,x_2)} = 2 \indic{\abs{2 x_2} > 2\sigma} + \frac{\abs{2 x_2}\indic{\abs{2 x_2} \leq 2\sigma}}{\sigma} \]
% Hence, we get that,
% \[ TV(D_1,D_2) = \Pr(\abs{2 x_2} > 2\sigma) + \frac{\Exp_{2 x_2 \sim D_x}[\abs{2 x_2}\indic{\abs{2 x_2} \leq 2\sigma}]}{2\sigma} \]

% We make a few observations,
% Consider a 1D-distribution, with the probability mass function given by
% \begin{align}
%   D_x(X = x) =  \begin{cases}
% \delta/2 , ~~ \text{if} ~~ x \in \{ -1/\delta^{1/4}, 1/\delta^{1/4} \} \\
% \frac{(1 - \delta)}{2\eta} ~~ \text{else if} ~~ x \in [-\eta,\eta], \\
% 0 ~~ \text{else} ~~
% \end{cases}
% \end{align}
% Consider two cases for $y|X=x$, in $D_1$, $y = x + \omega$, where $\omega \sim U(-\sigma,\sigma)$ independent of $x$ and for $D_2$, $y = -x + \omega$ for $\omega$ independent of $x$. Note that we'll put $\eta = \sigma \epsilon$, and $\delta = \epsilon$. From calculations in above page, this makes $TV$ between the two distributions $\epsilon$.  Now for this case,  
% \bit 
% \item $\Sigma^{\half} = \sqrt{\Exp[x^2]} = \delta^{1/4}$
% \[ \Exp[x^2] = \frac{(1-\delta)}{3} \eta^2 + \delta \cdot ( \frac{1}{\delta^{1/4}} )^2  = \frac{(1-\delta)}{3} \eta^2 + \sqrt{\delta} \]
% \item $\theta(D_1) - \theta(D_2) = 2$.
% \item So, our LHS is $\delta^{1/4}$. 
% \item $ \sigma \epsilon < \sigma < \frac{1}{\epsilon^{1/4}}$
% \item $1 = (\Exp[x_2^4])^{1/4} \leq c_4 \delta^{1/4}$. So our $C_4 = 1/\delta^{1/4}$.
% \eit 
% Now, let's look at our LHS,
% \begin{align*}
%     LHS & = \norm{\Sigma^{\half} \theta(D_1) - \theta(D_2)}{2} \\
%      & \textonTop{(1)}{=} \epsilon^{1/4} \\
%      & \textonTop{(2)}{\geq } \sigma \epsilon^{1/4} \epsilon^{1/4} \\
%      & \textonTop{(3)}{\geq} \frac{C_4}{C_4} \sigma \epsilon^{1/4} \epsilon^{1/4} \\
%      & \geq C_4 \sigma \epsilon^{3/4}
% \end{align*} 

Consider the means estimation example from LRV,

\begin{align}
   D_x(X = x) =  \begin{cases}
\delta , ~~ \text{if} ~~ x = \{ 1/\delta^{1/4} \} \\
\frac{(1 - \delta)}{2} ~~ \text{else if} ~~ x \in \{-1,1\}, \\
0 ~~ \text{else} ~~
\end{cases}
\end{align}
$D_1,D_2$ have the same marginal stated above. Note that the above distribution has variance $1+\sqrt{\delta}$, and fourth moment as $2$. 
For $D_1$ let $D_1(y|X = x) = x$. For $D_2$, 
let $D_2(y | X=x) = 0~if~x=1/\delta^{1/4}~else~x$. Then, $TV(D_1,D_2) = \delta$. 

Now, $\theta(D_1) = 1$, and $\theta(D_2) = \Exp[x^2]\inv \Exp[x y] = \frac{(1-\delta)}{1+\sqrt{\delta}}$. Hence, the diff between the two,
\[ \abs{\theta(D_1) - \theta(D_2) } = \frac{\delta + \sqrt{\delta}}{1 + \sqrt{\delta}} >> (\sqrt{\delta})  \]
